OpenOOD: Benchmarking Generalized Out-of-Distribution Detection

Out-of-distribution (OOD) detection is vital to safety-critical machine learning applications and has thus been extensively studied, with a plethora of methods developed in the literature. However, the field currently lacks a unified, strictly formulated, and comprehensive benchmark, which often results in unfair comparisons and inconclusive results. From the problem setting perspective, OOD detection is closely related to neighboring fields including anomaly detection (AD), open set recognition (OSR), and model uncertainty, since methods developed for one domain are often applicable to each other. To help the community to improve the evaluation and advance, we build a unified, well-structured codebase called OpenOOD, which implements over 30 methods developed in relevant fields and provides a comprehensive benchmark under the recently proposed generalized OOD detection framework. With a comprehensive comparison of these methods, we are gratified that the field has progressed significantly over the past few years, where both preprocessing methods and the orthogonal post-hoc methods show strong potential.

==> sections/4_codebase.tex <==
\section{Codebase Structure}
OpenOOD is a well-structured classification codebase tailored for methods under generalized OOD detection framework~\cite{yang2021generalized}.
As shown in Figure~\ref{fig:codebase}, we abstract a unified pipeline to meet the requirements of all state-of-the-art methods. Our pipeline consists of 6 main blocks including \texttt{Preprocessor}, \texttt{Dataloader}, \texttt{Network}, \texttt{Trainer}, \texttt{Evaluator}, and \texttt{Postprocessor}. 
While the \texttt{Dataloader} and \texttt{Evaluator} are mainly auxiliary blocks that do not need to be changed, a newly developed method only needs to account for modifications in the remaining 4 blocks by writing new Python classes.
The details of these blocks are explained below.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/codebase.pdf}
    \caption{\textbf{Structure diagram of OpenOOD codebase.} 
    OpenOOD is a well-structured, unified codebase that specialized for OOD detection tasks. This figure shows the main pipeline of OpenOOD. 
    To propose new OOD detection methods, developers can simply modify modules in colors.}
    \label{fig:codebase}
\end{figure}

\noindent\textbf{Preprocessor}\quad
The \texttt{Preprocessor} is used to process input images before feeding them into the network. With a single raw image as input, \texttt{Preprocessor} can produce output with either standard basic transformations such as Resize, Crop, Normalize, \etc, or curated data augmentation processes to support methods such as Cutpaste~\cite{cutpaste21cvpr}, PixMix~\cite{hendrycks2021pixmix}, and CutMix~\cite{cutmix19cvpr}.

\noindent\textbf{Network}\quad
To support methods with customized model structures, we provide \texttt{Network}, which require users to write an interface upon the standard backbones such as LeNet~\cite{lecun1998gradient}, ResNet18~\cite{he2016deep}, and ResNet50~\cite{he2016deep}. 
Example custom networks include ConfBranch~\cite{confbranch2018arxiv}, which adds another classifier from the penultimate layer to produce confidence apart from the main prediction. Other methods require unique \texttt{Network} include OpenGan~\cite{kong2021opengan} and DRAEM~\cite{zavrtanik2021draem}.

\noindent\textbf{Trainer}\quad
The \texttt{Trainer} component controls the training process. 
By taking the dataloader and network, \texttt{Trainer} takes charge of calculating loss functions. Methods with customized \texttt{Trainer} include ConfBranch~\cite{confbranch2018arxiv}, CutMix~\cite{cutmix19cvpr} and UDG~\cite{yang2021scood}.

\noindent\textbf{Evaluator and Postprocessor}\quad
\texttt{Postprocessor} takes the output from the network and return the prediction, score and ground truth for each data sample. Many methods only require a customized \texttt{Postprocessor} to fit in the code base include ODIN~\cite{odin18iclr}, MDS~\cite{mahananobis18nips} and KNN~\cite{sun2022knnood}.
\texttt{Postprocessor} is a built-in component of \texttt{Evaluator}, it utilize output from \texttt{Postprocessor} and calculate the accuracy and OOD score accordingly. All methods use BaseEvaluator for accuracy and OODEvaluator for OOD score.


==> sections/5_exploration.tex <==
\subsection{Further Exploration}

\paragraph{Are OOD Detectors Generalizable?}
\input{tables/fsood}
We split Table~\ref{T:main} vertically into several colored sections based on method type. Generally, the most effective methods lie in the category of model uncertainty. This group mainly contains simple and effective methods, such as the preprocessing methods such as PixMix~\cite{hendrycks2021pixmix} and CutMix~\cite{cutmix19cvpr}. Especially, PixMix gets 93.06\% on Near-OOD in CIFAR-10, which is the best among all the methods in this benchmark. They also ace in the most of other benchmarks. Similarly, other simple and effective methods such as Ensemble~\cite{deepensemble00iwmcs} and Mixup~\cite{mixup19nips} also show strong performance.

\paragraph{Are OOD Detectors Good Calibrators?}
For the block of OOD detection, we split it into two parts based on the necessity of extra data. 
By comparing UDG~\cite{yang2021scood} (the best from extra-data part) with KNN~\cite{sun2022knnood} (the best from extra data-free part), the advantage of UDG only lie in CIFAR-10 near-OOD, which does not meet the expectation as a large quantity of outlier exposure involved.
The extra data we use in this benchmark is the entire TinyImageNet training set, which is not purely OOD. In this case, among outlier-based methods only UDG has a reasonable performance considering other methods are not tuned to accept this kind of extra data we provide. For uncertainty methods, all methods listed here excluding TempScale require training, and their performance proves to be the largely better than other groups overall.

==> sections/8_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We build a well-structured codebase to comprehensively benchmark generalized OOD detection.}
  \item Did you describe the limitations of your work?
    \answerYes{See Conclusion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We cannot find any potential negative societal impacts in our work}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We read it and our codebase does not contain sensitive items}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{https://github.com/Jingkang50/OpenOOD}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Experiment Part}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We compare methods based on one pretrained model in our model zoo.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Experimental Section}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide the codebase link}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


